The Candidate Multi-Cut for Cell Segmentation

Two successful approaches for the segmentation of biomedical images are (1) the selection of segment candidates from a merge-tree, and (2) the clustering of small superpixels by solving a Multi-Cut problem. In this paper, we introduce a model that unifies both approaches. Our model, the Candidate Multi-Cut (CMC), allows joint selection and clustering of segment candidates from a merge-tree. This way, we overcome the respective limitations of the individual methods: (1) the space of possible segmentations is not constrained to candidates of a merge-tree, and (2) the decision for clustering can be made on candidates larger than superpixels, using features over larger contexts. We solve the optimization problem of selecting and clustering of candidates using an integer linear program. On datasets of 2D light microscopy of cell populations and 3D electron microscopy of neurons, we show that our method generalizes well and generates more accurate segmentations than merge-tree or Multi-Cut methods alone.

==> figures/results/table_abc.tex <==
\begin{table}[t]
\centering

\def\dataset{hela}
\def\datasetname{Dataset A}
\input{figures/results/quantitative}

\def\dataset{yeast}
\def\datasetname{Dataset B}
\input{figures/results/quantitative}

\def\dataset{pombe}
\def\datasetname{Dataset C}
\input{figures/results/quantitative}

\vspace{1mm}
\caption{Detection and segmentation results on datasets A, B, and C (light microscopy images). The best value in each column is highlighted.}
\vspace{-9mm}
\label{tab:results:abc}
\end{table}


==> figures/results/table_d.tex <==
\begin{table}[t]
\centering

\def\dataset{snemi_small-sp}
\def\datasetname{Dataset D}
\input{figures/results/quantitative_neurons}

\vspace{1mm}
\caption{Segmentation results on dataset D (electron microscopy volume). The best value in each column is highlighted.}
\vspace{-9mm}
\label{tab:results:d}
\end{table}


==> funkey/commands.tex <==
% This file provides some helpful macro commands.

\usepackage{todonotes}
\usepackage{xspace}

% todo-notes with a special color
\def\idea#1{{\todo[color=yellow!90!white]{#1}}\xspace}
\def\note#1{{\todo[color=orange!90!white]{#1}}\xspace}

% evaluate a mathematical expression #2 and assign the result to macro #1
\def\mathlet#1#2{\pgfmathparse{#2}\let#1\pgfmathresult}

% mark text as draft
\newenvironment{draft}{\color{red}}{}

% include a part of an image
\def\includetrimmed#1#2#3#4#5{%
  \includegraphics[%
    width=\samplewidth,%
    height=\sampleheight,%
    trim=#1px #2px #3px #4px,%
    clip]%
    {#5}%
}
\def\includesubimage#1#2#3#4#5{%
  \mathlet\l{#1}%
  \mathlet\t{#2}%
  \mathlet\r{\totalwidth-#3-#1}%
  \mathlet\b{\totalheight-#4-#2}%
  \includetrimmed{\l}{\b}{\r}{\t}{#5}%
}

% include files in a directory relative to current directory
\def\currentdir{.}%
\def\linput#1#2{%
  \begingroup%
  \edef\currentdir{\currentdir/#1}%
  \input{\currentdir/#2}%
  \endgroup%
}%


==> funkey/math.tex <==
% This file provides definitions of mathematical operators, symbols, and theorem 
% environments.


% defining equality
\newcommand{\define}{\stackrel{\text{\tiny def}}{=}}

% argmin, argmax
\newcommand{\argmin}[1]{\mathop{\arg\min}_{#1}\hspace{0.5em}}
\newcommand{\mmin}[1]{\mathop{\min}_{#1}\hspace{0.5em}}
\newcommand{\argmax}[1]{\mathop{\arg\max}_{#1}\hspace{0.5em}}
\newcommand{\mmax}[1]{\mathop{\max}_{#1}\hspace{0.5em}}

% const
\newcommand\const{\text{const}}

% transpose and inverse
\newcommand{\trans}[0]{{\sf T}}
\newcommand\inv{{-1}}

% annotations in equations
\newcommand{\annotation}[1]{& \text{{\small{#1}}}}

% function names
\newcommand\gauss{\mathcal{N}}

% ILP
%
% Usage:
%
% \beginilp
%   \objective{\
\def\beginilp{%
  \makeatletter
  \global\let\ilp@firstconstraint 0
  \global\def\ilp@name{}
  \makeatother
  % [name]{min,s.t.}[spacer]{objective,lhs}[rel][rhs][spacer][qualifier]
  \begin{IEEEeqnarray}{lr?rCl"l}
}
\def\name#1{%
  \makeatletter
  \global\def\ilp@name{#1:\;\;\;\;}
  \makeatother
}
\def\objective#1#2{%
  \makeatletter
  \global\let\ilp@firstconstraint 1
  \ilp@name
  \makeatother
  &
  #1
  &
  \IEEEeqnarraymulticol{4}{l}{#2}
}
\def\objectivecont#1{%
  \\
  &
  &
  \IEEEeqnarraymulticol{4}{l}{#1}
  \nonumber
}
\def\constraint#1#2#3#4{%
  \\
  &
  \makeatletter
  \if\ilp@firstconstraint 1 \text{s.t.} \fi
  \global\let\ilp@firstconstraint 0
  \makeatother
  &
  #1
  &
  #2
  &
  #3
  &
  #4
}
\def\endilp{%
  \end{IEEEeqnarray}
}


==> funkey/notation.tex <==
\usepackage{xifthen}

% isin version that expands its first argument
\newcommand*{\isinxp}[2]{\expandafter\isin\expandafter{#1}{#2}}

\newcommand{\mbb}[1]{{%
\ifthenelse{\isinxp{#1}{abcdefghijklmnopqrstuvxyz}}%
  {{\mathbf #1}}%
  {\boldsymbol #1}%
}}
\newcommand{\mup}[1]{{%
\ifthenelse{\isin{#1}{abcdefghijklmnopqrstuvxyzABCDEFGHIJKLMNOPQRSTUVXYZ}}%
  {\text{#1}}%
  {#1}%
}}

% vector
\newcommand{\vct}[1]{\protect\mbb{#1}}
% matrix
\newcommand{\mat}[1]{#1}
% set
\newcommand{\set}[1]{\protect\mbb{#1}}
% super-set
\newcommand{\sset}[1]{\boldsymbol{\mathcal{#1}}}
% random variable
\newcommand{\ran}[1]{#1}
% function
\newcommand{\fun}[1]{\mathrm{#1}}

% whole numbers
\newcommand{\whole}[0]{\mathbb{Z}}
% real numbers
\newcommand{\real}[0]{\mathbb{R}}
% natural numbers
\renewcommand{\natural}[0]{\mathbb{N}}

% abbreviations
\def\ie{{\it i.e.}}
\def\eg{{\it e.g.}}


==> funkey/tables.tex <==
% this file provides useful extensions to pgfplotstable:
%
% styles (found on stackexchange by user Jake):
%
%   highlight col max
%   highlight col min
%   highlight row max
%   highlight row min
% 
%   Usage:
%
%     \pgfplotstabletypeset[
%       highlight row max={<data>}{<row number>}
%     }{<data>}
%
%     or
%
%     \pgfplotstabletypeset[
%       highlight col max={<data>}{<column name>}
%     }{<data>}

\usepackage{pgfplotstable}
\usepackage{booktabs}
\usepackage{colortbl}

\newcommand{\findmax}[3]{%
    \pgfplotstablevertcat{\datatable}{#1}%
    \pgfplotstablecreatecol[%
    create col/expr={%%
    \pgfplotstablerow%
    }]{rownumber}\datatable%
    \pgfplotstablesort[sort key={#2},sort cmp={float >}]{\sorted}{\datatable}%%
    \pgfplotstablegetelem{0}{rownumber}\of{\sorted}%%
    \pgfmathtruncatemacro#3{\pgfplotsretval}%
    \pgfplotstableclear{\datatable}%
}%

\newcommand{\findmin}[3]{%
    \pgfplotstablevertcat{\datatable}{#1}%
    \pgfplotstablecreatecol[%
      create col/expr={%
    \pgfplotstablerow%
    }]{rownumber}\datatable%
    \pgfplotstablesort[sort key={#2},sort cmp={float <}]{\sorted}{\datatable}%
    \pgfplotstablegetelem{0}{rownumber}\of{\sorted}%%
    \pgfmathtruncatemacro#3{\pgfplotsretval}%
    \pgfplotstableclear{\datatable}%
}%

\pgfplotstableset{
  highlight content/.style={
    postproc cell content/.append style={
      @cell content/.add={$\bf}{$},
    }
  },
  highlight min content/.style={
    highlight content
  },
  highlight max content/.style={
    highlight content
  },
}

\pgfplotstableset{
    highlight col max/.code 2 args={
        \findmax{#1}{#2}{\maxval}
        \edef\setstyles{\noexpand\pgfplotstableset{
                every row \maxval\noexpand\space column #2/.style={
                    highlight max content
                }
            }
        }\setstyles
    },
    highlight col min/.code 2 args={
        \findmin{#1}{#2}{\minval}
        \edef\setstyles{\noexpand\pgfplotstableset{
                every row \minval\noexpand\space column #2/.style={
                    highlight min content
                }
            }
        }\setstyles
    },
    highlight row max/.code 2 args={
        \pgfmathtruncatemacro\rowindex{#2-1}
        \pgfplotstabletranspose{\transposed}{#1}
        \findmax{\transposed}{\rowindex}{\maxval}
        \edef\setstyles{\noexpand\pgfplotstableset{
                every row \rowindex\space column \maxval\noexpand/.style={
                    highlight max content
                }
            }
        }\setstyles
    },
    highlight row min/.code 2 args={
        \pgfmathtruncatemacro\rowindex{#2-1}
        \pgfplotstabletranspose{\transposed}{#1}
        \findmin{\transposed}{\rowindex}{\maxval}
        \edef\setstyles{\noexpand\pgfplotstableset{
                every row \rowindex\space column \maxval\noexpand/.style={
                    highlight min content
                }
            }
        }\setstyles
    },
}

\makeatletter%
\long\def\pgfplotstabletypeset@opt@collectarg[#1]#2{%
    \pgfplotstable@isloadedtable{#2}%
        {\pgfplotstabletypeset@opt@[#1]{#2}}%
        {\pgfplotstabletypesetfile@opt@[#1]{#2}}%
}%
\makeatother%


==> funkey/theorems.tex <==
% theorem environments

\usepackage{amsmath}
\usepackage{framed}
\usepackage[framed,thmmarks,amsmath]{ntheorem}

% general theorem style
\theoremstyle{plain}
\theorembodyfont{}
\def\theoremframecommand{\fcolorbox{black}{gray!20!white}}

\newshadedtheorem{theorem}{Theorem}[section]

\newshadedtheorem{lemma}[theorem]{Lemma}

\newshadedtheorem{proposition}[theorem]{Proposition}

\newshadedtheorem{corollary}[theorem]{Corollary}

\newshadedtheorem{definition}{Definition}[section]

{
\theoremstyle{nonumberplain}
\ifdefined\alternativetheoremsymbol
  \theoremsymbol{\alternativetheoremsymbol}
\else
  \theoremsymbol{\rule{1ex}{1ex}}
\fi
\theoremseparator{:}
\newtheorem{proof}{Proof}[section]
}


==> funkey/tikztension.tex <==
% This is the externalization variant of the tikztension, i.e., the one that 
% should be used to send to journals etc. It assumes that all graphics have been 
% generated in an appropriate format (pdf, ps, or eps) already. This is how you 
% can get rid of the tikz-dependence for publications.
\usepackage{graphics}

% single escape
%
% escapes a single character
\def\sesc#1{%
\if#1.-%   . -> -
\else%
\if#1=-%   = -> -
\else%
\if#1,-%   , -> -
\else%
\if#1/-%   / -> -
\else#1%
\fi%
\fi%
\fi%
\fi%
}

% denotes the end of the sequence to escape
\def\escnull{}

% escapes a sequence that ends with \escnull followed by \escend
\def\esc#1#2\escend{%
\ifx#1\escnull%
\else%
\sesc#1\esc#2\escend%
\fi%
}

% Escapes a string using the replacements in \sesc. Introduces no non-expandable 
% macros, i.e., the result can safely be used for filenames.
\def\escape#1{\esc#1\escnull\escend}

% #1 is the base name of the tikz file
% #2 is a string of PGF keys that are passed to \begin{tikzpicture}. It may 
% contain the special key /tikztension/define that defines empty macros. These 
% can be used as flags in the tikzimage via \ifdefined.
\newcommand{\includetikz}[2][]{%
  \def\graphicname{#2-\escape{#1}}%
  % include externalized graphic
  \includegraphics{\graphicname}%
}%


==> tikzstyles.tex <==
% empty export version of tikzstyles

